Combinatorial Bernoulli Factories

A Bernoulli factory is an algorithmic procedure for exact sampling of certain random variables having only Bernoulli access to their parameters. Bernoulli access to a parameter $p \in [0,1]$ means the algorithm does not know $p$, but has sample access to independent draws of a Bernoulli random variable with mean equal to $p$. In this paper, we study the problem of Bernoulli factories for polytopes: given Bernoulli access to a vector $x\in P$ for a given polytope $P\subset [0,1]^n$, output a randomized vertex such that the expected value of the $i$-th coordinate is \emph{exactly} equal to $x_i$. For example, for the special case of the perfect matching polytope, one is given Bernoulli access to the entries of a doubly stochastic matrix $[x_{ij}]$ and asked to sample a matching such that the probability of each edge $(i,j)$ be present in the matching is exactly equal to $x_{ij}$. We show that a polytope $P$ admits a Bernoulli factory if and and only if $P$ is the intersection of $[0,1]^n$ with an affine subspace. Our construction is based on an algebraic formulation of the problem, involving identifying a family of Bernstein polynomials (one per vertex) that satisfy a certain algebraic identity on $P$. The main technical tool behind our construction is a connection between these polynomials and the geometry of zonotope tilings. We apply these results to construct an explicit factory for the perfect matching polytope. The resulting factory is deeply connected to the combinatorial enumeration of arborescences and may be of independent interest. For the $k$-uniform matroid polytope, we recover a sampling procedure known in statistics as Sampford sampling.

==> tex_journal/open_journal.tex <==
\section{Open Questions and Future Directions}

\paragraph*{Strong Bernoulli factories for non-generic polytopes}

The most immediate open question is resolving the existence of strong Bernoulli factories for non-generic polytopes. In Section \ref{sec:impossibility_race_over_bernstein}, we have shown that no strong Bernoulli factory for the $k$-subset polytope $\Pnk$ can converge exponentially, thus ruling out our class of constructions. Do there exist strong Bernoulli factories for this polytope that do not converge exponentially? 

\begin{openproblem}
Does there exist a strong Bernoulli factory for the $k$-subset problem?
\end{openproblem}

Note that we can not even rule out the possibility that there exists a strong Bernoulli factory for $\Pnk$ which generates the same distribution over vertices as our current (non-strong) Bernoulli factory (i.e., returns vertex $v$ with probability $P_{v}(x)/\sum_{v'}P_{v'}(x)$). Such a factory, however, could not operate by running a Bernoulli race over Bernstein polynomials, and would have to simulate these rational functions in some other way. 

Conversely, our impossibility result (Theorem \ref{thm:impossibility}) currently only holds for the class of $k$-subset polytopes with $1 < k < n-1$. However, we know that some generic polytopes \emph{do} have strong Bernoulli factories (namely the $1$-subset and $n-1$-subset polytopes). Can we generalize this impossibility result to other generic polytopes, and understand when it is possible to implement strong Bernoulli factories?

\begin{openproblem}
Characterize the generic polytopes $\P$ for which there exists a strong Bernoulli factory that converges exponentially. 
\end{openproblem}

\paragraph{Explicit factories for other polytopes}

We have exhibited an explicit factory for the Birkhoff-von Neumann perfect matching polytope in Section \ref{sec:matching_factory}. This construction exhibits many nice combinatorial properties, such as being intricately connected to the enumeration of arborescences. It is natural to wonder whether such phenomena appear in factories for other combinatorial polytopes. One promising example is the \emph{flow polytope} (defined in the introduction), which like the matching polytope, is both integral and formed by interecting $[0, 1]^d$ with an affine subspace. 

\begin{openproblem}
Design an explicit Bernoulli factory for the flow polytope. 
\end{openproblem}

To help answer such questions, it would be useful to have a deeper understanding of how to construct factories for generic polytopes. While the perturbation-based method described in Section \ref{sec:generic} allowed us to numerically compute factories for instances of the matching polytope (which were then generalized by inspection), one could wish for a combinatorial algorithm that takes a generic factory and directly constructs a set $\U$ of valid partitions which lead to a correct Bernoulli factory. The arborescence-based factory for matchings could then hopefully be deduced directly from this algorithm.

\begin{openproblem}
Design a non-perturbation based method for constructing Bernoulli factories for non-generic polytopes. Is there a principled way to recover the arborescence-based factory for matchings from such a method?
\end{openproblem}

\subsection{$\epsilon$-Away Factories} If we only require the factory to hold $\epsilon$-away from the boundary...


\subsection{Sample complexity}

Given a factory $\mathcal{F}$ that terminates a.s. on $x$, it is natural to consider the quantity $C_{\mathcal{F}}(x) = \E[T_{\mathcal{F}}(x)]$, the expected number of coin flips required to simulate $\F$ on $x$. This represents the ``sample complexity'' of the factory, and is a major consideration when running such algorithms in practice.

For Bernoulli races over Bernstein polynomials, in each iteration we flip at most $2n$ coins and succeed with probability $(\sum_{v} P_{v}(x))/V$, and thus for our factories $\mathcal{F}$ for polytopes we have that

\begin{equation}
    C_{\mathcal{F}}(x) = \frac{2n|V|}{\sum_{v} P_{v}(x)}.
\end{equation}

The question remains: how large can this be? 
